Gradient Shaping for Multi-Constraint Safe Reinforcement Learning

Online safe reinforcement learning (RL) involves training a policy that maximizes task efficiency while satisfying constraints via interacting with the environments. In this paper, our focus lies in addressing the complex challenges associated with solving multi-constraint (MC) safe RL problems. We approach the safe RL problem from the perspective of Multi-Objective Optimization (MOO) and propose a unified framework designed for MC safe RL algorithms. This framework highlights the manipulation of gradients derived from constraints. Leveraging insights from this framework and recognizing the significance of \textit{redundant} and \textit{conflicting} constraint conditions, we introduce the Gradient Shaping (GradS) method for general Lagrangian-based safe RL algorithms to improve the training efficiency in terms of both reward and constraint satisfaction. Our extensive experimentation demonstrates the effectiveness of our proposed method in encouraging exploration and learning a policy that improves both safety and reward performance across various challenging MC safe RL tasks as well as good scalability to the number of constraints.

==> Texfiles/Schedule.tex <==
The remaining fields for this work to explore contain:
\begin{itemize}
    \item \textbf{Safety index learning scheme:} (i) The challenges for learning a valid safety index from the \textbf{offline dataset}. Some previous works~\citep{dawson2022safe, qin2021learning, qin2022sablas} proposed to online jointly learn the safety index (or, equivalently, CBF) and the RL policy to improve the performance. Although some works~\cite{liu2023safe} learned the safety index offline, they also face problems such as over-conservativeness. (ii) Loss function~(\ref{equ: loss function for safety index})  design for the safety index learning. It is crucial for us to get a valid safety index that ensures a both forward-invariant and non-conservative safe set for the subsequent policy learning.
    \item \textbf{Constraint encoding for policy update :} Based on recent work results~\citep{liu2023datasets} and current experiments, the off-policy update formulation (\ref{equ: estep_objective}) requires a non-conservative constraint that ensures there exists at least one feasible solution for the training stability. Consequently, we may need a relaxed formulation for the policy update.
\end{itemize}
\textbf{Future Plan:}
\begin{itemize}
    \item Determine the setting for this work. For example, whether to train the safety index online or offline; and whether to jointly learn the safety index and policy or not.
    \item Experiment setup. Targeting tasks: Circle tasks in Bullet-Safety-Gym~\citep{gronauer2022bullet}, and Goal/Button tasks in the Safety-Gym~\citep{ray2019benchmarking}, Safety-Gymnasium~\citep{Safety-Gymnasium}, or GUARD~\citep{zhao2023guard}.
    \item Baseline comparison. Targeting comparing algorithms: (1) Model-Free Off-Policy Safe RL such as CVPO~\citep{liu2022constrained} 
    (2) Model-Free On-Policy Safe RL such as PPO-Lag, TRPO-Lag \citep{stooke2020responsive} (3) Model-Based State-wise Safe RL algorithm such as TRPO-FAC \citep{ma2021feasible}, TRPO-SL \citep{dalal2018safe}.
\end{itemize}
